A Simple and Generic Framework for Feature Distillation via Channel-wise Transformation

Knowledge distillation is a popular technique for transferring the knowledge from a large teacher model to a smaller student model by mimicking. However, distillation by directly aligning the feature maps between teacher and student may enforce overly strict constraints on the student thus degrade the performance of the student model. To alleviate the above feature misalignment issue, existing works mainly focus on spatially aligning the feature maps of the teacher and the student, with pixel-wise transformation. In this paper, we newly find that aligning the feature maps between teacher and student along the channel-wise dimension is also effective for addressing the feature misalignment issue. Specifically, we propose a learnable nonlinear channel-wise transformation to align the features of the student and the teacher model. Based on it, we further propose a simple and generic framework for feature distillation, with only one hyper-parameter to balance the distillation loss and the task specific loss. Extensive experimental results show that our method achieves significant performance improvements in various computer vision tasks including image classification (+3.28% top-1 accuracy for MobileNetV1 on ImageNet-1K), object detection (+3.9% bbox mAP for ResNet50-based Faster-RCNN on MS COCO), instance segmentation (+2.8% Mask mAP for ResNet50-based Mask-RCNN), and semantic segmentation (+4.66% mIoU for ResNet18-based PSPNet in semantic segmentation on Cityscapes), which demonstrates the effectiveness and the versatility of the proposed method. The code will be made publicly available.

==> alpha.tex <==
\begin{table}[t]
    \centering
  \begin{tabular}{c|cc}
    \toprule
     different $\alpha$ & mIoU  & - \\
     \midrule
     1e-5 & 73.49 & - \\
     2e-5 & 74.51 & - \\
     3e-5 & 74.42 & - \\ 
     4e-5 & 73.70 & - \\
     5e-5 & 73.12 & - \\
    \bottomrule
  \end{tabular}
  \caption{Different $\alpha$.}
  \vspace{-0.05in}
  \label{table:alpha}
\end{table}

==> analysis_kl.tex <==
\begin{figure}
    \centering
    \includegraphics[width = 0.45\textwidth]{figs/kl_div.pdf}
    \vspace{-4mm}
    \caption{Following the method used in \cite{shu2021cwd}, we calculate the KL divergence between the student model (Faster RCNN-ResNet50) and the teacher model (CascadeMask RCNN ResNeXt10) on different FPN levels. There is no correlation between feature similarity and model performance. Our student has the worst similarity to teacher but achieves best mAP on COCO dataset.}
    % it is not the case that the more similar the student model and the teacher model are, the better performance the student model can achieve.
    
    \label{fig:kl_div_mlp}
\end{figure}

==> different_mask_ratio.tex <==
\begin{figure}
    \centering
    \includegraphics[width = 0.45\textwidth]{differnt_mask_ratio_.pdf}
    \vspace{-4mm}
    \caption{different mask ratio}
    
    
    \label{fig:kl_div_mlp}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> radar.tex <==
\begin{figure}
    \centering
    \includegraphics[width = 0.45\textwidth]{radar_.pdf}
    \caption{
    Our simple method achieves state-of-the-art performance on a wide range of vision tasks compared to other task-specific or general methods under the same setting. We report the average improvement in Top-1 accuracy, bbox mAP, mask mAP, and mIoU for classification, object detection, instance segmentation, and semantic segmentation, respectively. We calculate the performance improvement across all configurations in our paper, and we evaluate the simplicity of our method using the number of hyper-parameters as a metric (less is better).
    }
    \label{fig:radar}
\end{figure}
